Uncertainty Quantification with Statistical Guarantees in End-to-End Autonomous Driving Control

Deep neural network controllers for autonomous driving have recently benefited from significant performance improvements, and have begun deployment in the real world. Prior to their widespread adoption, safety guarantees are needed on the controller behaviour that properly take account of the uncertainty within the model as well as sensor noise. Bayesian neural networks, which assume a prior over the weights, have been shown capable of producing such uncertainty measures, but properties surrounding their safety have not yet been quantified for use in autonomous driving scenarios. In this paper, we develop a framework based on a state-of-the-art simulator for evaluating end-to-end Bayesian controllers. In addition to computing pointwise uncertainty measures that can be computed in real time and with statistical guarantees, we also provide a method for estimating the probability that, given a scenario, the controller keeps the car safe within a finite horizon. We experimentally evaluate the quality of uncertainty computation by several Bayesian inference methods in different scenarios and show how the uncertainty measures can be combined and calibrated for use in collision avoidance. Our results suggest that uncertainty estimates can greatly aid decision making in autonomous driving.

==> Sections/oldrelatedworks.tex <==
\section{Related Works}


\ifthenelse{\boolean{showoldcomments}}{\RM{Everything below, work in progress!}}{}

% General structure:
    % paragraph on deterministic models (end-to-end)
        % why we are better: uncertainty is useful yo
    % paragraph (possibly two? lots of content here) on bayesian and probabilistic models
        % address each paper individually on why we are better (possibly only consider smaller models, do not provide actual guarantees)
    % paragraph on safety certification for autonomous driving
        % again, address individually

% End-to-end controllers (deterministic models)
End-to-end controllers for autonomous driving are a popular research topic due to their independence from complex, specifically coded scenarios, instead allowing the network to define its own features based on training. Examples of such controllers include CNNs,  \cite{chen2017end} and \cite{bojarski2017explaining}, fully convolutional networks with long short term memory (FCN-LSTM), \cite{xu2017end}.
%, are trained on real-world driving data for lane keeping with the input to the network being a pre-processed image, and the output a continuous steering angle (a regression problem). 
%PilotNet \cite{bojarski2017explaining}, the network we modify and use to evaluate the framework defined in this paper, is another prominent example of an end-to-end controller for autonomous driving.
While all of these controllers performed well in testing, they are deterministic, and as such, do not give any information on how certain the controller is in its prediction. Prior to Bayesian deep learning, there is a rich literature on detecting anomalies from sensor output \cite{isermann1984faultdetection}; however, these methods deal with when sensor outputs deviate from normal ranges and do not detect when the sensors are operating perfectly, but the situation itself is anomalous or unsafe. For this, quantification of model and data uncertainty, extracted from BNNs, can be used \cite{kendall2017uncertainties}. 
% end sentence about how our framework takes uncertainty into account? too obvious? No- this should be done in the methods section

% bayesian and probabilistic models - TODO i like 5,6,7,8 ordering, but perhaps move 2 and 9?
%paper 9 - Spatial Uncertainty Sampling for End-to-End Control - I believe this is just pointwise again, please correct me if i missed something! Yes this is just pointwise. So we dont need to discuss it in too much detail.
% I am moving it for
%edit counter-factuals part

%paper 5 & 6
Several works that deploy small vehicles have dealt with the issue outlined above, in controlled conditions. In \cite{lee2018ensemble}, an ensemble of BNNs over different modalities (stereo imaging and GPS) are used in order to drive a 1:5 scale car autonomously around an oval track. The authors show how uncertainty can be used in order to distrust the decisions of models which are using noisy data, thus leading to safer driving. Further, in \cite{kahn2017uncertainty}, they use bootstrapping and dropout in order to generate uncertainty estimates which allow an RC car or quad-rotor drone to predict and avoid collisions. Our work improves upon these papers by testing with both realistic scale, and realistic conditions, which allows us to better estimate how uncertainty improves safety than in the limited scopes described here.%\LL{Also we can stress that we have bounds to quantify the predictions}

%papers 7 & 8 & 2
\ifthenelse{\boolean{showoldcomments}}{\RM{TODO: strengthen part on why we are better than these three papers}}{}

Beyond these simplified domains important work is being done in scaling end-to-end BNN models to real world test cases. In \cite{amini2019variational}, the authors use a variational neural network in order to incorporate GPS and image data to make predictions about long term navigation and localization. \cite{huang2019uncertainty} looks at using uncertainty from a variational neural network to produce both a distribution of possible future trajectories of a car at an intersection, and a confidence estimate for varying time horizons, with the final goal of augmenting the result of this with a physics-based predictor using confidence estimates. Additionally, in \cite{feng2018towards} BNNs are used on real-world LiDAR data in order to more safely localize objects.

%transition to safety certifications for autonomous driving?
%paper 1 & paper 3
%\cite{amini2018learning} \LL{THis paper does not use BNNs. } proposes a new BNN based approach that learns a continuous control probability distribution, and from this, gathers steering control options and bounds for these. The authors then demonstrate how these bounds can be used in a parallel autonomy setting, with the car intervening when the human driver attempts to steer outside of the computed steering bounds. In \cite{blake2018efficient}, the authors present methods for calculating the probabilistic risk of collision for a given trajectory, assuming a distribution over the pose of objects in the environment. While these two papers work towards safety in autonomous driving, they do not provide bounds or guarantees on the safety of the system as a whole, which is a major contribution of the framework presented here. 
\ifthenelse{\boolean{showoldcomments}}{\RM{reword last sentence}.}{}


%In \cite{amini2018spatial}, the authors use 2D spatial dropout to generate accurate uncertainty estimates from a deep Bayesian network for end-to-end autonomous vehicle control. Their method has a lower mean uncertainty error that for traditional, element-wise dropout, and they demonstrate that their uncertainty estimates can be used to develop a shared controller to fuse a human's action with the network's output according to those estimates.


We further the investigation into safe deployment of BNNs as end-to-end controllers by scaling exact and approximate inference techniques to realistic simulators. This allows for the contextualization of point-wise uncertainty estimates and enables their use in real-time decision making. Understanding that uncertainty increases for certain inputs (as in \cite{amini2019variational} \cite{feng2018towards} \cite{huang2019uncertainty}) is important insofar as it encourages the use of uncertainty during deployment; however, evaluating the uncertainty in a point-wise (per image) fashion does not allow us to reason about emergent properties of the incorporation of uncertainty and their safety \cite{cardelli2019robustness}. In order to create safe plans for autonomous vehicles that incorporate uncertainty, we must evaluate the fundamental impact of decisions which are made on the bases of uncertainty (e.g. slowing down when uncertain, or returning control to the user).  

\ifthenelse{\boolean{showoldcomments}}{\RM{how to phrase this? something like "the framework described in this paper uses uncertainty in paths rather than pointwise" but way better}.}{}
%safety certs for autonomous driving
%paper 10

Finally, \cite{quilbeuf2018statistical} looks at using statistical model checking (SMC) to evaluate the probability of two different subsystems of an autonomous vehicle controller (therefore not an end-to-end controller) meeting specific key performance indicators (KPIs). Examples of these KPIs include the number of stops in the critical area of a junction being less than a given threshold, and the acceleration of the car being less than a given threshold. Although the results of this paper demonstrated a high probability of meeting the KPIs, the simulator used was very basic (no scenery, only a simple junction, cars look like boxes etc), and the controller used was not end-to-end, and therefore does not have the benefits described in this work.
